Reporting Revenge Porn: a Preliminary Expert Analysis

In our research, we focus on the response to the non-consensual distribution of intimate or sexually explicit digital images of adults, also referred as revenge porn, from the point of view of the victims. In this paper, we present a preliminary expert analysis of the process for reporting revenge porn abuses in selected content sharing platforms. Among these, we included social networks, image hosting websites, video hosting platforms, forums, and pornographic sites. We looked at the way to report abuse, concerning both the non-consensual online distribution of private sexual image or video (revenge pornography), as well as the use of deepfake techniques, where the face of a person can be replaced on original visual content with the aim of portraying the victim in the context of sexual behaviours. This preliminary analysis is directed to understand the current practices and potential issues in the procedures designed by the providers for reporting these abuses.

==> future.tex <==
\section{Future Work}\label{sec:future}
This preliminary expert evaluation permits us to extend the analysis with a qualitative research approach. We plan to identify a heterogeneous set of users, composed of people having different ages, genders, educational backgrounds and technological expertise, for testing and analysing their behaviours by reporting a given media, on dedicated webpages, where the different report modalities will be replicated. 















